SAW: A Tool for Safety Analysis of Weakly-hard Systems

We introduce SAW, a tool for safety analysis of weakly-hard systems, in which traditional hard timing constraints are relaxed to allow bounded deadline misses for improving design flexibility and runtime resiliency. Safety verification is a key issue for weakly-hard systems, as it ensures system safety under allowed deadline misses. Previous works are either for linear systems only, or limited to a certain type of nonlinear systems (e.g., systems that satisfy exponential stability and Lipschitz continuity of the system dynamics). In this work, we propose a new technique for infinite-time safety verification of general nonlinear weakly-hard systems. Our approach first discretizes the safe state set into grids and constructs a directed graph, where nodes represent the grids and edges represent the reachability relation. Based on graph theory and dynamic programming, our approach can effectively find the safe initial set (consisting of a set of grids), from which the system can be proven safe under given weakly-hard constraints. Experimental results demonstrate the effectiveness of our approach, when compared with the state-of-the-art. An open source implementation of our tool is available at https://github.com/551100kk/SAW. The virtual machine where the tool is ready to run can be found at https://www.csie.ntu.edu.tw/~r08922054/SAW.ova.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> sections/rebuttal.tex <==
\section{Response}

Reiterate the contribution and novelty (For the last reviewer).

We would like to first thank all the reviewers for their constructive and insightful comments. We will make sure to address the typos and other minor inconsistencies in the revision. We want to reiterate that the contribution of this tool lies on both the discretization-based framework and the graph-theory based algorithms in each phase of the tool, rather than restricting to a specific new dynamic programming algorithm. As far as we know, this tool is the first tool for verifying weakly-hard systems. In the following, we clarify the main concerns from reviewers.

Review questions:

R2-Q1: Scalability analysis of real-time complex systems.

Our tool consists of two parts: a discretization-based framework and a back-end reachability analysis technique, which are both sensitive to the dimension of the dynamical systems. For the discretization-based framework, a potential improvement is to more intelligently partition the state space via heuristic methods, e.g. the grids that are closer to the equilibrium point can be set larger to reduce the number of overall grids. For the reachability analysis tool, Flow* constructs flowpipes based on Taylor expansion for the nonlinear dynamic, which also suffers from curse of dimensionality. Despite this, the tool provides an insight on verifying weakly-hard systems. Further improvement is needed for handling large scale systems.


R3-Q1: Soundness of the back-end reachability analysis tool.

The soundness of the back-end reachability analysis technique is indeed important for the overall soundness of the tool. Thus we choose Flow*, which leverages the flowpipe construction based on Taylor expansion for the nonlinear dynamic. It is not a simulation-based approach and it computes the valid overapproximation of the reachable set. Thus the soundness is guaranteed.

R7-Q1: Concerns on novelty and contribution.

Please refer to the contribution clarification in the first paragraph.


Artifact review questions:

R4-Q1 and R5-Q1: One-dimension abstraction is not provided.

This tool does not include one-dimension abstraction. The experimental results of one-dimension abstraction are from \cite{huang2019formal}.

R5-Q2: The details of packages and connection.

Most of the packages are the dependencies of Flow*. Gnuplot is used to plot the result svg in this tool. 

R5-Q3: Experiments are only explored for an only small finite time ($\leq$ 2) and small dimensional systems ($\leq$ 2).

The experiments are all for infinite verification problem. All the experiments are collected from the state-of-the-art related works. As aforementioned for R2-Q1, the current technique could indeed be inefficient for high-dimensional systems due to the curse of dimensionality, but it shows a promising direction for verifying weakly-hard systems and there are potential methods for improving its efficiency. 

R6-Q1: Some inconsistencies in the model definition/codes, output figures. Minor problems on Table, Listing.

We apologize for the inconsistencies. Most of those can be fixed by modifying the parameters in the model file. Other issues are clarified as follow:

(1) Figures : The output figure for each run of the tool can be found in the same directory as output.svg. 

(2) SHA1: The correct SHA1 sum is written in the README.md in the Github repository. The one in the VM is not updated since we cannot know the hash until we have generated the OVA file.

(3) Runtime: The runtime could change depending on the CPU and memory status for both the guest and the host operating systems. We can interpret the relative runtime comparing to the model with the different parameters.

R6-Q2: For Ex.5, How to verify $Gamma_1$ is $[-1.56, 1.32]$ when $step\_size$ 0.1.

The tool will output the safe initial region in the standard output for one-dimension model. The result for Ex.5 can be reproduced by running the program with the example model file, example/model5.txt.

R6-Q3: Explain the results of the case $(m,K) = (2,9)$ and $(m,K) = (3,9)$.

Formally, $(m,K) = (2,9)$ and $(m,K) = (3,9)$ represent that among 9 consecutive sampling periods, at most 2 and 3 deadline misses would occur, respectively. Intuitively, making system safe under the constraint $(m,K) = (3,9)$ is more difficult since more deadline misses may happen -- This is reflected in its smaller safe initial region shown in the paper.







